Tight Sample Complexity of Learning One-hidden-layer Convolutional Neural Networks

We study the sample complexity of learning one-hidden-layer convolutional neural networks (CNNs) with non-overlapping filters. We propose a novel algorithm called approximate gradient descent for training CNNs, and show that, with high probability, the proposed algorithm with random initialization grants a linear convergence to the ground-truth parameters up to statistical precision. Compared with existing work, our result applies to general non-trivial, monotonic and Lipschitz continuous activation functions including ReLU, Leaky ReLU, Sigmod and Softplus etc. Moreover, our sample complexity beats existing results in the dependency of the number of hidden nodes and filter size. In fact, our result matches the information-theoretic lower bound for learning one-hidden-layer CNNs with linear activation functions, suggesting that our sample complexity is tight. Our theoretical analysis is backed up by numerical experiments.

==> non-iterative.tex <==

\subsection{Direction estimation}
In this section we consider a simple algorithm to estimate the direction of parameter vectors $\wb_*$ and $\vb_*$. 

\begin{algorithm}[h]
\caption{Direction Estimation for Non-overlapping CNN} \label{alg:NOCNN}
\begin{algorithmic}
\REQUIRE Training data $\{(\xb_i,y_i)\}_{i=1}^n$.
\FOR{$j=1,2,3,\ldots, r$}
\STATE $\hat{\ub}_j = \frac{1}{n} \sum _{i=1}^n y_i \Pb_j \xb_i$
\ENDFOR
\STATE $\hat{\wb} = \frac{1}{r}\sum_{j=1}^r \hat{\ub}_j $
\ENSURE $\hat{\wb}$.
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[h]
\caption{Direction Estimation for Non-overlapping CNN, 2 layers} \label{alg:NOCNN2layer}
\begin{algorithmic}
\REQUIRE Training data $\{(\xb_i,y_i)\}_{i=1}^n$.
\STATE $\hat{\ub}_1 = \frac{1}{n} \sum _{i=1}^n y_i \Pb_1 \xb_i$
\FOR{$j=1,2,3,\ldots, r$}
\STATE $\hat{\ub}_j = \frac{1}{n} \sum _{i=1}^n y_i \Pb_j \xb_i$
\ENDFOR
\STATE Set $l = \argmax_j \|\hat{\ub}_j\|_2$
\FOR{$j=1,2,3,\ldots, r$}
\STATE $a_j = \mathrm{sign}(\hat{\ub}_l^\top \hat{\ub}_j) $
\ENDFOR
\STATE $\tilde{\wb} = \hat{\ub}_l $, $\tilde{\vb} = (a_1\|\hat{\ub}_1\|_2,\ldots, a_r\|\hat{\ub}_r\|_2)^\top$
%\STATE $\tilde{\wb} = \frac{1}{r}\sum_{j=1}^r a_j\hat{\ub}_j $, $\tilde{\vb} = (a_1\|\hat{\ub}_1\|_2,\ldots, a_r\|\hat{\ub}_r\|_2)^\top$.
%\STATE $(b,c) = \argmin_{b,c\in \{\pm 1\}} \sum_{i=1}^n \big[y_i - b\sum_{j=1}^r\tilde{v}_j \sigma(c\tilde{\wb}^\top \Pb_j \xb_i)\big]^2$
%\STATE $\hat{\wb} = c\tilde{\wb}$, $\hat{\vb} = b\tilde{\vb}$
%\ENSURE $\hat{\wb}$, $\hat{\vb}$.
\ENSURE $\tilde{\wb}$, $\tilde{\vb}$
\end{algorithmic}
\end{algorithm}
\CC{use $\tilde v_j$ instead of $\tilde \vb_j$ because it's a scalar}






\begin{algorithm}[h]
\caption{Direction Estimation for Overlapping CNN} \label{alg:OCNN}
\begin{algorithmic}
\REQUIRE Training data $\{(\xb_i,y_i)\}_{i=1}^n$.
\STATE $\tilde{\wb} =  \frac{1}{n} \sum _{i=1}^n y_i \Pb_1 \xb_i$
\STATE $\hat{w}_1 = \tilde{w}_1$
\FOR{$l=2,3,\ldots, k$}
\STATE $\hat{w}_l = \tilde{w}_{l} -\tilde{w}_{l-1}$
\ENDFOR
\ENSURE $\hat{\wb} = (\hat{w}_1,\ldots, \hat{w}_k)^\top$.
\end{algorithmic}
\end{algorithm}


\iffalse

\begin{algorithm}[h]
\caption{Direction Estimation for Non-overlapping CNN} \label{alg:NOCNN}
\begin{algorithmic}
\REQUIRE Training data $\{(\xb_i,y_i)\}_{i=1}^n$.
\FOR{$j=1,2,3,\ldots, r$}
\STATE $\hat{\ub}_j = \frac{1}{n} \sum _{i=1}^n y_i \Pb_j \xb_i$
\ENDFOR
\STATE $\hat{\wb} = \frac{1}{r}\sum_{j=1}^r \hat{\ub}_j $, $\hat{\vb} = (\|\hat{\ub}_1\|, \|\hat{\ub}_2\|, \ldots, \|\hat{\ub}_r\|)$
\ENSURE $\hat{\wb}$, $\hat{\vb}$.
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[h]
\caption{Direction Estimation for overlapping CNN} \label{alg:NOCNN}
\begin{algorithmic}
\REQUIRE Training data $\{(\xb_i,y_i)\}_{i=1}^n$.
\FOR{$j=1,2,3,\ldots, r$}
\STATE $\hat{\ub}_j = \frac{1}{n} \sum _{i=1}^n y_i \Pb_j \xb_i$
\ENDFOR
\STATE $\hat{\wb} = \frac{1}{r}\sum_{j=1}^r \hat{\ub}_j $, $\hat{\vb} = (\|\hat{\ub}_1\|, \|\hat{\ub}_2\|, \ldots, \|\hat{\ub}_r\|)$
\ENSURE $\hat{\wb}$, $\hat{\vb}$.
\end{algorithmic}
\end{algorithm}

\fi

\iffalse
\begin{algorithm}[h]
\caption{Direction Estimation for Non-overlapping CNN} \label{alg:NOCNN}
\begin{algorithmic}
\REQUIRE Training data $\{(\xb_i,y_i)\}_{i=1}^n$.
\STATE Randomly split the training data into $T$ subsets, each with size $n/T$.
\FOR{$t=1,2,3,\ldots, T$}
\STATE $\wb_{t} = \wb_{t-1} - \eta\nabla\hcL_{S_t}(\wb_{t-1})$
\ENDFOR
\ENSURE $\wb_T$.
	\end{algorithmic}
\end{algorithm}


It is worth noting that the key difference between the resampling version and vanilla gradient descent is that we split the whole sample $\{(\xb_i,y_i)\}_{i=1}^n$ into $T$ subsets, where $T$ is the total number of iterations in gradient descent,  and we use one fresh subset for each iteration. This resampling procedure ensures the independence between $\wb_{t-1}$ and the subsample  $\{(\xb_i,y_i), i\in S_t\}$ used for updating $\wb_{t-1}$, which is essential for later analysis. More specifically, we first randomly split the training sample $\{(\xb_i,y_i)\}_{i=1}^n$ into $T$ different subsets: $\{(\xb_i,y_i), i\in S_1\},\{(\xb_i,y_i),i\in S_2\}, \ldots \{(\xb_i,y_i),i\in S_T\}$, where the cardinality of $S_t$ is $|S_t|=n/T$, and we only use the subset $\{(\xb_i,y_i), i\in S_t\}$ for the 
update in the $t$-th iteration. Furthermore, we write $\hcL_{S_t}(\wb)$ as the empirical loss function with respect to the subsample used in the $t$-th iteration, and give the formal definition of $\hcL_{S_t}(\wb)$ as follows
\begin{align*}
\hcL_{S_t}(\wb) = \frac{1}{2|S_t|} \sum_{i\in S_t} \big(\sigma(\wb^\top\xb_i) - y_i\big)^2.
\end{align*}
\fi

\section{Main Theory}

\begin{definition}
We define the function $\gamma(h) :=  \EE_{z\sim N(0,1)}[\sigma(hz)z]$ for any $h\in\RR$.
\end{definition}

\CC{add assumptions}
\begin{assumption}\label{assump:Lipschitz}
The activation function $\sigma$ is $L$-Lipschitz for some constant $L>0$ such that 
\begin{align*}
    |\sigma(z_1)-\sigma(z_2)|\leq L|z_1-z_2|, \text{ for all }z_1,z_2\in\RR. 
\end{align*}
\end{assumption}






The following lemma is given by \cite{zhong2017recovery}. 

\begin{lemma}[\cite{zhong2017recovery}]\label{lemma:momentcalculation}
For any $(\xb,y)$ generated by the model in \eqref{eq:cnndef}, we have
\begin{align*}
    \EE_{(\xb,y)\sim \cD}[y\cdot \xb] = \frac{\gamma(\|\wb^*\|_2)}{\|\wb^*\|_2}\sum_{i=1}^r \Pb_i^\top \wb^*,
\end{align*}
\end{lemma}





The following lemma characterizes an important property of Algorithm \ref{alg:NOCNN}, which estimates the direction of $\wb^*$.
\begin{lemma}
For the estimator $\hat \wb$ output by Algorithm \ref{alg:NOCNN}, we have
\begin{align*}
    \EE[\hat\wb] = \frac{\gamma(\|\wb^*\|_2)}{\|\wb^*\|_2}\wb^*.
\end{align*}
where $\gamma(h) :=  \EE_{z\sim N(0,1)}[\sigma(hz)z]$.
\end{lemma}

\subsection{Non-overlapped CNN}

\begin{theorem}\label{lemma:directionconcentrationNO}
If the activation function $\sigma$ is $L$- Lipschitz with $L>0$, with probability at least $1-\delta$, the output of Algorithm~\ref{alg:NOCNN} satisfies
\begin{align*}
    \bigg\| \hat{\wb} - \frac{\gamma(\|\wb^*\|_2)}{\|\wb^*\|_2} \wb^* \bigg\|_2 \leq  C\Bigg\{ M   \sqrt{\frac{2rk\log(2n^2r)\log(60r/\delta)}{n}}
    + [r\sigma(0)
    + \nu]\sqrt{\frac{k\log(30/\delta)}{nr}} \Bigg\},
\end{align*}
where $M = \max\{ L\|\wb^*\|_2,\|\wb^*\|_2^2\} $ and $C$ is an absolute constant. Moreover, we have
\begin{align*}
    \bigg\la \frac{\hat{\wb}}{\|\hat{\wb}\|_2}, \frac{\wb^*}{\|\wb^*\|_2} \bigg\ra \geq 1- \frac{C'}{\gamma^2(\|\wb^*\|_2)}\Bigg\{ M   \sqrt{\frac{2rk\log(2n^2r)\log(60r/\delta)}{n}}
    + [r\sigma(0)
    + \nu]\sqrt{\frac{k\log(30/\delta)}{nr}} \Bigg\}^2,
\end{align*}
where $C'$ is an absolute constant.
\end{theorem}

\CC{add a remark on the assumption}
\begin{remark}

\end{remark}
\begin{proof}[Proof of Theorem~\ref{lemma:directionconcentrationNO}]
Let $\cN_{1/2}$ be a $1/2$-net covering the unit Euclidean sphere $S^{k-1}$, then by Lemma~5.2 in \cite{vershynin2010introduction}, we have 
$
|\cN_{1/2}| \leq 5^k.
$
For any vector $\zb\in \cN_{1/2}$, we have
\begin{align*}
    \zb^\top \hat{\wb} = \frac{1}{nr}  \sum_{j=1}^r\sum_{i=1}^n y_i \cdot \zb^\top\Pb_j\xb_i.
\end{align*}
Plugging \eqref{eq:cnndef} into the equation above gives
\begin{align*}
    \zb^\top \hat{\wb} =  \frac{1}{n} \sum_{j=1}^r  \sum_{i=1}^n  \Bigg[\sum_{j'=1}^r \sigma(\wb^{*\top} \Pb_{j'} \xb_{i}) + \epsilon_{i}\Bigg]\cdot\zb^\top\Pb_j\xb_i =  I_1 + I_2 + I_3 ,
\end{align*}
where
\begin{align*}
   &I_1  = \frac{1}{nr} \sum_{j=1}^r \sum_{j'=1}^r \sum_{i=1}^n [\sigma(\wb^{*\top}  \Pb_{j'} \xb_{i})-\sigma(0)]\cdot\zb^\top\Pb_j\xb_i,\\
   &I_2 = \frac{1}{nr} \sum_{j=1}^r \sum_{i=1}^n r\sigma(0)\cdot\zb^\top\Pb_j\xb_i,\\
   &I_3 = \frac{1}{nr} \sum_{j=1}^r\sum_{i=1}^n \epsilon_{i}\cdot\zb^\top\Pb_j\xb_i.
\end{align*}

It is easy to see that $\EE(I_1) = \EE(\zb^\top \hat{\wb}) $ and $\EE(I_2) = \EE(I_3) =0$. We now analyze the concentration of the three terms. 

\noindent \textbf{Concentration of $I_1$}. We reorganize the sum as follows.
\begin{align*}
    I_1 =  \frac{1}{n\sqrt{r}} \sum_{j'=1}^r \sum_{i=1}^n    [\sigma(\wb^{*\top}  \Pb_{j'} \xb_{i})-\sigma(0)]\cdot \frac{1}{\sqrt{r}} \sum_{j=1}^r \zb^\top\Pb_j\xb_i.
\end{align*}
Let 
\begin{align}\label{eq:def_Vi}
    U_{ij'} = \sigma(\wb^{*\top}  \Pb_{j'} \xb_{i})-\sigma(0),~ V_i = \frac{1}{\sqrt{r}} \sum_{j=1}^r \zb^\top\Pb_j\xb_i,~ i=1,\ldots,n.
\end{align}
By Lipschitz condition, for $i=1,\ldots, n$ we have $|U_{ij'}| \leq   L|\wb^{*\top} \Pb_{j'} \xb_{i}|$. Therefore by Lemma~\ref{lemma:Gaussiantail} and union bound, with probability at least $1-\eta$, $|U_{ij'}| \leq R$
for all $i=1,\ldots, n$ and $j'=1,\ldots, r$, where $ R = L\|\wb^*\|_2  \sqrt{2\log(2nr/\eta)}$. 
Moreover, $V_1,\ldots, V_n$ are i.i.d. standard normal random variables. 
Let $\hat{U}_{ij'} = U_{ij'}\ind (|U_{ij'}| \leq R) $, then we have
\begin{align}\label{eq:decomp_I1}
    \Bigg| \frac{1}{n} \sum_{i=1}^n U_{ij'} V_i - \EE(U_{1j'} V_1) \Bigg| \leq & \Bigg| \frac{1}{n} \sum_{i=1}^n (U_{ij'} - \hat{U}_{ij'}) V_i \Bigg| + \Bigg| \frac{1}{n} \sum_{i=1}^n \hat{U}_{ij'} V_i - \EE(\hat{U}_{1j'} V_1)\Bigg| \notag\\ 
    &\qquad+ \big| \EE(U_{1j'} V_1) - \EE(\hat{U}_{1j'} V_1)  \big|.
\end{align}
We now proceed to bound the three terms on the right-hand side above. By definition of $R$, with probability at least $1-\eta$ the first term on the right hand side of \eqref{eq:decomp_I1} vanishes for all $j'=1,\ldots,r$ and $\zb\in \cN_{1/2}$. For the second term, by Lemma~\ref{lemma:subgaussianproduct} we have
\begin{align*}
    \| \hat{U}_{ij'} V_i \|_{\psi_1} \leq C_1R
\end{align*}
for some absolute constant $C_1$. Therefore by Proposition~5.16 in \cite{vershynin2010introduction}, with probability at least $1-\delta/6$, we have
\begin{align*}
    \Bigg| \frac{1}{n} \sum_{i=1}^n (U_{ij'} - \hat{U}_{ij'}) V_i \Bigg| \leq C_2 R\sqrt{\frac{k\log(60r/\delta)}{n}}
\end{align*}
\CC{should the left hand side be the second term?}for all $j'=1,\ldots, r$ and $\zb\in \cN_{1/2}$, where $C_2$ is an absolute constant.
For the third term, we have
\begin{align*}
    \big| \EE(U_{1j'} V_1) - \EE(\hat{U}_{1j'} V_1)  \big| \leq \EE \big(\big| U_{1j'} - \hat{U}_{1j'}\big|\cdot V_1 \big) = \EE (| U_{1j'}|\cdot \ind (U_{1j'} > R)\cdot V_1 ).
\end{align*}
Applying Cauchy-Schwarz inequality gives
\begin{align*}
    \big| \EE(U_{1j'} V_1) - \EE(\hat{U}_{1j'} V_1)  \big| \leq C_3\sqrt{\eta}\|\wb^*\|_2^2, 
\end{align*}
where $C_3$ is an absolute constant. Therefore, with probability at least $1-\eta - \delta/6$, we have
\begin{align*}
    \Bigg| \frac{1}{n} \sum_{i=1}^n U_{ij'} V_i - \EE(U_{1j'} V_1) \Bigg| \leq C_2 L\|\wb^*\|_2  \sqrt{\frac{2k\log(2nr/\eta)\log(60r/\delta)}{n}} + C_3\sqrt{\eta}\|\wb^*\|_2^2
\end{align*}
for all $j'=1,\ldots, r$. Setting $\eta = \min\{\delta/6, 1/n\}$ and plugging the inequality above into the definition of $I_1$, we have that with probability at least $1-\delta/3$,
%\begin{align*}
%    \Bigg| \frac{1}{n} \sum_{i=1}^n U_{ij'} V_i - \EE(U_{1j'} V_1) \Bigg| \leq C_2 L\|\wb^*\|_2  \sqrt{\frac{2k\log(2n^2r)\log(60r/\delta)}{n}} + C_3\|\wb^*\|_2^2\frac{1}{\sqrt{n}}.
%\end{align*}
%Therefore we have
\begin{align}\label{eq:directionconcentrationNO1}
    |I_1 - \EE[\zb^\top \hat{\wb}] | \leq C_2 L\|\wb^*\|_2  \sqrt{\frac{2rk\log(2n^2r)\log(60r/\delta)}{n}} + C_3\|\wb^*\|_2^2\sqrt{\frac{r}{n}}
\end{align}
for all $\zb \in \cN_{1/2}$.





\iffalse
\begin{align*}
    U^{(j)}_{ij'} &= [\sigma(\wb^{*\top}  \Pb_{j'} \xb_{i}) - \sigma(0)] \cdot \zb^\top\Pb_j\xb_i,\\
    V^{(j)}_{ij'} &= \sigma(0) \cdot \zb^\top\Pb_j\xb_i.
\end{align*}

By Lemma~\ref{lemma:subgaussianproduct} and (5.15) in \cite{vershynin2010introduction} as an equivalent definition of $\psi_1$-norm, we have 
$$
\|U^{(j)}_{ij'}\|_{\psi_1} \leq L\|\wb^{*\top} \Pb_{j'} \xb_{i} \cdot  \zb^\top\Pb_j\xb_i \|_{\psi_1} \leq  C_1L\|\wb^{*}\|,
$$
where $C_1$ is an absolute constant. Applying Proposition~5.16 in \cite{vershynin2010introduction} to $\{U^{(j)}_{ij'}\}$, we have that with probability at least $1-\delta/3$, we have
\begin{align*}
    \Bigg|\frac{1}{n} \sum_{i=1}^n U^{(j)}_{ij'} - \delta_{j,j'}\EE(\zb^\top \hat{\wb})\Bigg| \leq C_2L\|\wb^*\| \sqrt{\frac{k\log[30r^2/\delta]}{n}}
\end{align*}
for all $j,j'\in [r]$ and all $\zb \in \cN_{1/2}$, 
where $C_2$ is an absolute constant. Therefore with probability at least $1-\delta/3$, we have
\begin{align}\label{eq:directionconcentrationNO2}
    \Big|I_1^{(j)} - \EE(\zb^\top \hat{\wb})\Big| \leq C_2Lr\|\wb^*\| \sqrt{\frac{k\log[30r^2/\delta]}{n}}
\end{align}
for all $j\in [r]$ and all $\zb \in \cN_{1/2}$.
\fi

\noindent \textbf{Concentration of $I_2$}. Since $\cI_{1},\ldots,\cI_{r}$ do not overlap, $I_2$ is an average of $nr$ independent Gaussian random variables. For any $\zb \in\cN_{1/2}$, the $\psi_2$-norm of $\zb^\top\Pb_j\xb_i$ is the $\psi_2$-norm of standard normal random variables. Therefore by Proposition~5.10 in \cite{vershynin2010introduction}, with probability at least $1-\delta/3$, we have
\begin{align}\label{eq:directionconcentrationNO2}
    |I_2|\leq C_4\sigma(0)\sqrt{\frac{rk\log(15e/\delta)}{n}},
\end{align}
where $C_4$ is an absolute constant.


\noindent \textbf{Concentration of $I_3$}.
We have 
\begin{align*}
    I_3= \frac{1}{rn} \sum_{j=1}^r \sum_{i=1}^n \epsilon_{i}\cdot\zb^\top\Pb_j\xb_i.
\end{align*}
Since $\cI_{1},\ldots,\cI_{r}$ do not overlap, for $j'\neq j$, $\Pb_{j'} \xb_{i}$ and $\Pb_{j} \xb_{i}$ contains different entries of $\xb_i$. Therefore, let $v_1,\ldots, v_n \sim N(0,1)$ be i.i.d. standard normal random variables, then we have \CC{$v_i$ are the same as $V_i$ defined in \eqref{eq:def_Vi}}
\begin{align*}
    I_3 = \frac{1}{n\sqrt{r}}  \sum_{i=1}^n \epsilon_{i}\cdot \sum_{j=1}^r\frac{1}{\sqrt{r}}\zb^\top\Pb_j\xb_i \overset{d}{=} \frac{1}{n\sqrt{r}}  \sum_{i=1}^n \epsilon_{i}\cdot v_i.
\end{align*}
Moreover we have $\|\epsilon_{i}\cdot v_i\|_{\psi_1} \leq C_4 \nu$ for some absolute constant $C_5$. By Proposition~5.16 in \cite{vershynin2010introduction}, with probability at least $1-\delta/3$, we have
\begin{align}\label{eq:directionconcentrationNO3}
    |I_3|  \leq C_6\nu \sqrt{\frac{k\log(30/\delta)}{nr}}
\end{align}
for all $\zb\in \cN_{1/2}$, where $C_6$ is an absolute constant. 
By \eqref{eq:directionconcentrationNO1}, \eqref{eq:directionconcentrationNO2},\eqref{eq:directionconcentrationNO3} and the definition of $\hat{\wb}$, we have
\begin{align*}
    |\zb^\top (\hat{\wb} - \EE[\hat{\wb}])| \leq &  C_2 L\|\wb^*\|_2  \sqrt{\frac{2rk\log(2n^2r)\log(60r/\delta)}{n}} + C_3\|\wb^*\|_2^2\sqrt{\frac{r}{n}} \\ 
    &\qquad+ C_4\sigma(0)\sqrt{\frac{k\log(15e/\delta)}{nr}}
    + C_6 \nu\sqrt{\frac{k\log(30/\delta)}{nr}}
\end{align*}
for all $\zb\in \cN_{1/2}$. Now by Lemma~5.3 in \cite{vershynin2010introduction} and Lemma~\ref{lemma:momentcalculation}, we have that with probability at least $1-\delta$,
\begin{align*}
    \bigg\| \hat{\wb} - \frac{\gamma(\|\wb^*\|)}{\|\wb^*\|} \wb^* \bigg\|_2 \leq & C\Bigg[ L\|\wb^*\|_2  \sqrt{\frac{2rk\log(2n^2r)\log(60r/\delta)}{n}} + \|\wb^*\|_2^2\sqrt{\frac{r}{n}} \\ 
    &\qquad+ \sigma(0)\sqrt{\frac{rk\log(15e/\delta)}{n}}
    + \nu\sqrt{\frac{k\log(30/\delta)}{nr}} \Bigg],
\end{align*}
where $C$ is an absolute constant. The first result of Lemma~\ref{lemma:directionconcentrationNO} directly follows the inequality above.
The second result of Lemma~\ref{lemma:directionconcentrationNO} follows by Lemma~\ref{lemma:distance2innerproduct}.
\end{proof}





















\subsection{Non-overlapped CNN, 2 layer}
In this section we consider the convolutional neural network with unknown second layer parameters $\vb^*$.
\CC{use $v_j^*$ instead of $\vb_j^*$ because it's a scalar}
\begin{align}\label{eq:cnndef2layer}
    y_{i} = \sum_{j=1}^r  v^*_j\sigma(\wb^{*\top} \Pb_{j} \xb_{i}) + \epsilon_{i},
\end{align}

\CC{how about the estimation error bound of $\wb$?}

\CC{The following bound is a bound on the bias?}


\begin{lemma}\label{lemma:uhatexpectationNO2layer} 
For any $(\xb,y)$ generated by the model in \eqref{eq:cnndef2layer}, we have
\begin{align*}
    \EE (\hat{\ub}_j) = \frac{\gamma(\|\wb^*\|_2)}{\|\wb^*\|_2} v^*_j \wb^*,~j=1,\ldots,r.
\end{align*}
\end{lemma}


\begin{lemma}\label{lemma:uhatconcentrationNO2layer}
In Algorithm~\ref{alg:NOCNN2layer}, with probability at least $1-\delta$ we have
\begin{align*}
   \|\hat{\ub}_j - \EE[\hat{\ub}_j] \|_2 \leq C \Bigg\{ M\|\vb^*\|_1   \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} +  [ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}} \Bigg\},
\end{align*}
for all $j=1,\ldots,r$, where $M = \max\{ L\|\wb^*\|_2,\|\wb^*\|_2^2\} $ and $C$ is an absolute constant.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:uhatconcentrationNO2layer}]
Let $\cN_{1/2}$ be a $1/2$-net covering the unit Euclidean sphere $S^{k-1}$, then by Lemma~5.2 in \cite{vershynin2010introduction}, we have 
$
|\cN_{1/2}| \leq 5^k.
$
For any vector $\zb\in \cN_{1/2}$, we have
\begin{align*}
    \zb^\top \hat{\ub}_j = \frac{1}{n} \sum_{i=1}^n y_i \cdot \zb^\top\Pb_j\xb_i,~j=1,\ldots,r.
\end{align*}
We next proof the concentration result for $\hat{\ub}_1$, and the proofs for $\hat{\ub}_2,\ldots, \hat{\ub}_r$ are exactly the same. Plugging \eqref{eq:cnndef2layer} into the equation above gives
\begin{align*}
    \zb^\top \hat{\ub}_1 =  \frac{1}{n}  \sum_{i=1}^n  \Bigg[\sum_{j'=1}^r v^*_{j'}\sigma(\wb^{*\top} \Pb_{j'} \xb_{i}) + \epsilon_{i}\Bigg]\cdot\zb^\top\Pb_1\xb_i =  I_1 + I_2 ,
\end{align*}
where
\begin{align*}
   &I_1  = \frac{1}{n} \sum_{j'=1}^r \sum_{i=1}^n [v^*_{j'}\sigma(\wb^{*\top}  \Pb_{j'} \xb_{i})-\sigma(0)]\cdot\zb^\top\Pb_1\xb_i,\\
   &I_2 = \frac{1}{n} \sum_{i=1}^n \Bigg[\sigma(0)\cdot\sum_{j'=1}^r v^*_{j'} + \epsilon_{i} \Bigg] \cdot\zb^\top\Pb_1\xb_i,\\
\end{align*}
It is easy to see that $\EE(I_1) = \EE(\zb^\top \hat{\wb}) $ and $\EE(I_2) =0$. We now analyze the concentration of the two terms. 

\noindent \textbf{Concentration of $I_1$}.
Let 
$$
U_{ij'} = \sigma(\wb^{*\top}  \Pb_{j'} \xb_{i})-\sigma(0),~ V_i = \zb^\top\Pb_j\xb_i,~ i=1,\ldots,n.
$$
By Lipschitz condition, for $i=1,\ldots, n$ we have $|U_{ij'}| \leq   L|\wb^{*\top} \Pb_{j'} \xb_{i}|$. Therefore by Lemma~\ref{lemma:Gaussiantail} and union bound, with probability at least $1-\eta$, $|U_{ij'}| \leq R$
for all $i=1,\ldots, n$ and $j'=1,\ldots, r$, where $ R = L\|\wb^*\|_2  \sqrt{2\log(2nr/\eta)}$. 
Moreover, $V_1,\ldots, V_n$ are i.i.d. standard normal random variables. 
Let $\hat{U}_{ij'} = U_{ij'}\ind (|U_{ij'}| \leq R) $, then we have
\begin{align*}
    \Bigg| \frac{1}{n} \sum_{i=1}^n U_{ij'} V_i - \EE(U_{1j'} V_1) \Bigg| \leq & \Bigg| \frac{1}{n} \sum_{i=1}^n (U_{ij'} - \hat{U}_{ij'}) V_i \Bigg| + \Bigg| \frac{1}{n} \sum_{i=1}^n \hat{U}_{ij'} V_i - \EE(\hat{U}_{1j'} V_1)\Bigg| \\ 
    &\qquad+ \big| \EE(U_{1j'} V_1) - \EE(\hat{U}_{1j'} V_1)  \big|.
\end{align*}
We now proceed to bound the three terms on the right-hand side above. By definition of $R$, with probability at least $1-\eta$ the first term vanishes for all $j'=1,\ldots,r$ and $\zb\in \cN_{1/2}$. For the second term, by Lemma~\ref{lemma:subgaussianproduct} we have
\begin{align*}
    \| \hat{U}_{ij'} V_i \|_{\psi_1} \leq C_1R
\end{align*}
for some absolute constant $C_1$. Therefore by Proposition~5.16 in \cite{vershynin2010introduction}, with probability at least $1-\delta/(4r)$, we have
\begin{align*}
    \Bigg| \frac{1}{n} \sum_{i=1}^n (U_{ij'} - \hat{U}_{ij'}) V_i \Bigg| \leq C_2 R\sqrt{\frac{k\log(40r^2/\delta)}{n}}
\end{align*}
for all $j'=1,\ldots, r$ and $\zb\in \cN_{1/2}$, where $C_2$ is an absolute constant.
For the third term, we have
\begin{align*}
    \big| \EE(U_{1j'} V_1) - \EE(\hat{U}_{1j'} V_1)  \big| \leq \EE \big(\big| U_{1j'} - \hat{U}_{1j'}\big|\cdot V_1 \big) = \EE (| U_{1j'}|\cdot \ind (U_{1j'} > R)\cdot V_1 ).
\end{align*}
Applying Cauchy-Schwarz inequality gives
\begin{align*}
    \big| \EE(U_{1j'} V_1) - \EE(\hat{U}_{1j'} V_1)  \big| \leq C_3\sqrt{\eta}\|\wb^*\|_2^2, 
\end{align*}
where $C_3$ is an absolute constant. Therefore, with probability at least $1-\eta - \delta/(4r)$, we have
\begin{align*}
    \Bigg| \frac{1}{n} \sum_{i=1}^n U_{ij'} V_i - \EE(U_{1j'} V_1) \Bigg| \leq C_2 L\|\wb^*\|_2  \sqrt{\frac{2k\log(2nr/\eta)\log(40r^2/\delta)}{n}} + C_3\sqrt{\eta}\|\wb^*\|_2^2
\end{align*}
for all $j'=1,\ldots, r$. Setting $\eta = \min\{\delta/(4r), 1/n\}$ and plugging the inequality above into the definition of $I_1$, we have that with probability at least $1-\delta/(2r)$,
\begin{align}\label{eq:directionconcentrationNO2layer1}
    |I_1 - \EE[\zb^\top \hat{\wb}] | \leq C_2 Lr\|\wb^*\|_2 \|\vb^*\|_1  \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} + C_3\|\wb^*\|_2^2\|\vb^*\|_1 \frac{1}{\sqrt{n}}
\end{align}
for all $\zb \in \cN_{1/2}$. 

\noindent \textbf{Concentration of $I_2$}.
By Lemma~\ref{lemma:subgaussianproduct} we have $\|[\sigma(0)+\epsilon_{i}]\cdot \zb^\top\Pb_1\xb_i\|_{\psi_1} \leq C_4 [ \|\vb^*\|_1 \sigma(0) + \nu ]$ for some absolute constant $C_4$. By Proposition~5.16 in \cite{vershynin2010introduction}, with probability at least $1-\delta/(2r)$, we have
\begin{align}\label{eq:directionconcentrationNO2layer2}
    |I_3|  \leq C_5[ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}}
\end{align}
for all $\zb\in \cN_{1/2}$, where $C_5$ is an absolute constant. 
By \eqref{eq:directionconcentrationNO2layer1}, \eqref{eq:directionconcentrationNO2layer2}, and the definition of $\hat{\ub}_1$, with probability at least $1 - \delta/r$, we have
\begin{align*}
    |\zb^\top (\hat{\ub}_1 - \EE[\hat{\ub}_1])| \leq & C_2 L\|\wb^*\|_2\|\vb^*\|_1   \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} + C_3\|\wb^*\|_2^2\|\vb^*\|_1 \frac{1}{\sqrt{n}} \\
    &+ C_5[ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}}
\end{align*}
for all $\zb\in \cN_{1/2}$. Now by Lemma~5.3 in \cite{vershynin2010introduction}, we have
\begin{align*}
    \|\hat{\ub}_1 - \EE[\hat{\ub}_1] \|_2 \leq C \Bigg\{ M\|\vb^*\|_1   \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} +  [ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}} \Bigg\},
\end{align*}
where $M = \max\{ L\|\wb^*\|_2,\|\wb^*\|_2^2\} $. 
By the same proof, we have that with probability at least $1-\delta$,
\begin{align*}
   \|\hat{\ub}_j - \EE[\hat{\ub}_j] \|_2 \leq C \Bigg\{ M\|\vb^*\|_1   \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} +  [ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}} \Bigg\},
\end{align*}
for all $j=1,\ldots,r$. This completes the proof. 
\end{proof}







\begin{lemma}\label{lemma:recoversignNO2layer}
There exists an absolute constant $C$ such that with probability at least $1-\delta$, for any $j=1,\ldots,r$, if 
\begin{align*}
    |v^*_j| \gamma(\|\wb^*\|_2)> C\Bigg\{ M\|\vb^*\|_1   \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} +  [ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}} \Bigg\},
\end{align*}
where $M = \max\{ L\|\wb^*\|_2,\|\wb^*\|_2^2\} $, then $a_j = \sign(v^*_l v^*_j)$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:recoversignNO2layer}]
Let $\zeta = \gamma(\|\wb^*\|_2)$ and
\begin{align*}
    \eta = C'\Bigg\{ M\|\vb^*\|_1   \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} +  [ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}} \Bigg\},
\end{align*}
where $C'$ is the absolute constant given by Lemma~\ref{lemma:uhatconcentrationNO2layer}. We set $C = 5C'$. Then by Lemma~\ref{lemma:uhatexpectationNO2layer} and Lemma~\ref{lemma:uhatconcentrationNO2layer}, with probability at least $1-\delta$ we have
\begin{align*}
   \big|\|\hat{\ub}_j \|_2 - \zeta v^*_j| \big| \leq \eta,~j=1,\ldots,r.
\end{align*}
By the definition of $l$, we have
\begin{align*}
    \zeta|v^*_j|\leq \big| \zeta v^*_j - \|\hat{\ub}_j \|_2\big| + \|\hat{\ub}_l \|_2 \leq \eta + \big| \zeta v^*_l - \|\hat{\ub}_l \|_2\big| + \zeta|v^*_l| \leq 2\eta + \zeta |v^*_l|.
\end{align*}
By the inequality above and the assumption that $\zeta |v^*_j| >5\eta$, we have $\zeta |v^*_l| > \eta$. Plugging this into the inequality above again to cancel $eta$ gives $|v^*_j| \leq 3 |v^*_l|$. 
Moreover, we have
\begin{align*}
    \big|\hat{\ub}_l^\top \hat{\ub}_j - \EE(\hat{\ub}_l^\top) \EE(\hat{\ub}_j) \big| &\leq \big|\hat{\ub}_l^\top \hat{\ub}_j - \hat{\ub}_l^\top \EE(\hat{\ub}_j) \big| + \big| \hat{\ub}_l^\top \EE(\hat{\ub}_j) - \EE(\hat{\ub}_l^\top) \EE(\hat{\ub}_j) \big|\\
    &\leq \eta \big[\|\hat{\ub}_l\|_2 + \|\EE(\hat{\ub}_1)\|_2\big] \\
    &\leq   \eta \big[\zeta (| v^*_l| + | v^*_j|) + \eta \big]\\
    &< 5\zeta \eta |v^*_l|
\end{align*}
On the other hand, we have
$\EE(\hat{\ub}_1^\top) \EE(\hat{\ub}_j) = \zeta^2v^*_1v^*_j$, and
\begin{align*}
    \big|\hat{\ub}_l^\top \hat{\ub}_j - \EE(\hat{\ub}_l^\top) \EE(\hat{\ub}_j) \big| <5\zeta \eta |v^*_l| < \zeta^2|v^*_l||v^*_j| = \big|\EE(\hat{\ub}_1^\top) \EE(\hat{\ub}_j)\big|.
\end{align*}
The inequality above implies that $a_j = \sign(\hat{\ub}_l^\top \hat{\ub}_j) = \sign[\EE(\hat{\ub}_1^\top) \EE(\hat{\ub}_j)] = \sign(v^*_l v^*_j)$.
\end{proof}



















\begin{lemma}\label{lemma:vtildeNO2layer}
In Algorithm~\ref{alg:NOCNN2layer}, with probability at least $1-\delta$ we have
\begin{align*}
    \big| \tilde{v}_j - &\sign( v^*_l)\gamma(\|\wb^*\|)  v^*_j \big| \\
    &\leq C \Bigg\{ M\|\vb^*\|_1   \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} +  [ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}} \Bigg\},
\end{align*}
where $M = \max\{ L\|\wb^*\|_2,\|\wb^*\|_2^2\} $ and $C$ is the absolute constant.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:vtildeNO2layer}]
Let $$
\eta = C' \Bigg\{ M\|\vb^*\|_1   \sqrt{\frac{2k\log(2n^2r)\log(40r^2/\delta)}{n}} +  [ \|\vb^*\|_1 \sigma(0) + \nu ] \sqrt{\frac{k\log(20r/\delta)}{n}} \Bigg\},
$$
where $C'$ is the absolute constant given by Lemma~\ref{lemma:uhatconcentrationNO2layer}. Denote $\zeta = \gamma(\|\wb^*\|_2)$. Then by Lemma~\ref{lemma:uhatexpectationNO2layer} and Lemma~\ref{lemma:uhatconcentrationNO2layer}, with probability at least $1-\delta$ we have
\begin{align}\label{eq:vtildeNO2layer1}
   \big|\|\hat{\ub}_j \|_2 - \zeta v^*_j| \big| \leq \eta,~j=1,\ldots,r.
\end{align}
Let $C''$ be the absolute constant introduced by Lemma~\ref{lemma:recoversignNO2layer} and $c = C''/C'$. For each $v^*_j$, $j=1,\ldots,r$,
we consider two cases.

\noindent (i) If $|v^*_j| \leq c\zeta$, then by \eqref{eq:vtildeNO2layer1} we have
\begin{align*}
    |\tilde{v}_j| = \|\hat{\ub}_j \|_2 \leq (c+1)\eta,
\end{align*}
and therefore 
\begin{align*}
    \big| \tilde{v}_j - \sign( v^*_l)\zeta  v^*_j \big| \leq |\tilde{v}_j| + \zeta | v^*_j| \leq (2c+1) \eta.
\end{align*}


\noindent (ii) If $|v^*_j| > C\eta /\zeta$, by Lemma~\ref{lemma:recoversignNO2layer}, with probability at least $1-\delta$ we have $a_j = \sign(v^*_l v^*_j)$.
Therefore by \eqref{eq:vtildeNO2layer1} we have
\begin{align*}
    \big| \tilde{v}_j - \sign( v^*_l)\zeta  v^*_j \big| = \big| \sign(v^*_l v^*_j) \|\hat{\ub}_j\|_2 - \sign( v^*_l)\zeta  v^*_j \big| = \big|  \|\hat{\ub}_j\|_2 - \zeta  |v^*_j| \big| \leq \eta.
\end{align*}
This completes the proof.
\end{proof}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







\subsection{Overlapped CNN}

%\CC{add overlapping cases}




\begin{lemma}\label{lemma:directionconcentrationOwtildeexpectation}
In Algorithm~\ref{alg:OCNN}, we have
\CC{change $l'$ to something else, for example, $j$ or $s$}
\begin{align*}
    \tilde{\wb}_l = \frac{\gamma(\|\wb^*\|_2)}{\|\wb^*\|_2} \sum_{s=1}^l \wb^*_{s},~l=1,\ldots,k
\end{align*}
\end{lemma}
\begin{proof}

\end{proof}





\begin{lemma}\label{lemma:directionconcentrationOwtilde}
With probability at least $1-\delta$, we ahve
\begin{align*}
    \| \tilde{\wb} - \EE(\tilde{\wb}) \|_2 \leq & C\Bigg[M' r  \sqrt{\frac{2k\log(2n^2r)\log(40r/\delta)}{n}} +  \nu \sqrt{\frac{k\log(20/\delta)}{n}} \Bigg],
\end{align*}
where $M' = \max\{ L[\|\wb^*\|_2 + |\sigma(0)|], \|\wb^*\|_2^2 + \sigma^2(0) \}$, and $C$ is an absolute constant.
\end{lemma}





















\begin{proof}[Proof of Lemma~\ref{lemma:directionconcentrationOwtilde}]
Let $\cN_{1/2}$ be a $1/2$-net covering the unit Euclidean sphere $S^{k-1}$, then by Lemma~5.2 in \cite{vershynin2010introduction}, we have 
$
|\cN_{1/2}| \leq 5^k.
$
For any vector $\zb\in \cN_{1/2}$, we have
\begin{align*}
    \zb^\top \tilde{\wb} = \frac{1}{n} \sum_{i=1}^n y_i \cdot \zb^\top\Pb_1\xb_i.
\end{align*}
Plugging \eqref{eq:cnndef} into the equation above gives
\begin{align*}
    \zb^\top \tilde{\wb} =  \frac{1}{n}  \sum_{i=1}^n  \Bigg[\sum_{j=1}^r \sigma(\wb^{*\top} \Pb_{j} \xb_{i}) + \epsilon_{i}\Bigg]\cdot\zb^\top\Pb_1\xb_i =  I_1 + I_2 + I_3 ,
\end{align*}
where
\begin{align*}
   &I_1  = \frac{1}{n} \sum_{j=1}^r \sum_{i=1}^n \sigma(\wb^{*\top}  \Pb_{j} \xb_{i})\cdot\zb^\top\Pb_1\xb_i,\\
   &I_2 = \frac{1}{n} \sum_{i=1}^n \epsilon_{i}\cdot\zb^\top\Pb_j\xb_i.
\end{align*}

It is easy to see that $\EE(I_1) = \EE[\zb^\top \tilde{\wb}] $ and $\EE(I_2) =0$. We now analyze the concentration of the two terms. 

\noindent \textbf{Concentration of $I_1$}. 
Let 
$$
U_{ij} = \sigma(\wb^{*\top}  \Pb_{j} \xb_{i}),~ V_i = \zb^\top\Pb_1\xb_i,~ i=1,\ldots,n.
$$
By Lipschitz condition, for $i=1,\ldots, n$ we have $|U_{ij}| \leq   L|\wb^{*\top} \Pb_{j} \xb_{i}| + |\sigma(0)|$. Therefore by Lemma~\ref{lemma:Gaussiantail} and union bound, with probability at least $1-\eta$, $|U_{ij'}| \leq R$
for all $i=1,\ldots, n$ and $j=1,\ldots, r$, where $ R = L\|\wb^*\|_2  \sqrt{2\log(2nr/\eta)} + |\sigma(0)|$. 
Moreover, $V_1,\ldots, V_n$ are i.i.d. standard normal random variables. 
Let $\hat{U}_{ij} = U_{ij}\ind (|U_{ij}| \leq R) $, then we have
\begin{align*}
    \Bigg| \frac{1}{n} \sum_{i=1}^n U_{ij} V_i - \EE(U_{1j} V_1) \Bigg| \leq & \Bigg| \frac{1}{n} \sum_{i=1}^n (U_{ij} - \hat{U}_{ij}) V_i \Bigg| + \Bigg| \frac{1}{n} \sum_{i=1}^n \hat{U}_{ij} V_i - \EE(\hat{U}_{1j} V_1)\Bigg| \\ 
    &\qquad+ \big| \EE(U_{1j} V_1) - \EE(\hat{U}_{1j} V_1)  \big|.
\end{align*}
We now proceed to bound the three terms on the right-hand side above. By definition of $R$, with probability at least $1-\eta$ the first term vanishes for all $j=1,\ldots,r$ and $\zb\in \cN_{1/2}$. For the second term, by Lemma~\ref{lemma:subgaussianproduct} we have
\begin{align*}
    \| \hat{U}_{ij} V_i \|_{\psi_1} \leq C_1R
\end{align*}
for some absolute constant $C_1$. Therefore by Proposition~5.16 in \cite{vershynin2010introduction}, with probability at least $1-\delta/4$, we have
\begin{align*}
    \Bigg| \frac{1}{n} \sum_{i=1}^n (U_{ij} - \hat{U}_{ij'}) V_i \Bigg| \leq C_2 R\sqrt{\frac{k\log(40r/\delta)}{n}}
\end{align*}
for all $j=1,\ldots, r$ and $\zb\in \cN_{1/2}$, where $C_2$ is an absolute constant.
For the third term, we have
\begin{align*}
    \big| \EE(U_{1j} V_1) - \EE(\hat{U}_{1j} V_1)  \big| \leq \EE \big(\big| U_{1j} - \hat{U}_{1j}\big|\cdot V_1 \big) = \EE (| U_{1j}|\cdot \ind (U_{1j} > R)\cdot V_1 ).
\end{align*}
Applying Cauchy-Schwarz inequality gives
\begin{align*}
    \big| \EE(U_{1j} V_1) - \EE(\hat{U}_{1j} V_1)  \big| \leq C_3\sqrt{\eta}[\|\wb^*\|_2^2 + \sigma^2(0)], 
\end{align*}
where $C_3$ is an absolute constant. Therefore, with probability at least $1-\eta - \delta/4$, we have
\begin{align*}
    \Bigg| \frac{1}{n} \sum_{i=1}^n U_{ij} V_i - \EE(U_{1j} V_1) \Bigg| \leq C_2 R  \sqrt{\frac{k\log(40r/\delta)}{n}} + C_3\sqrt{\eta}\cdot \big(\|\wb^*\|_2^2 + \sigma^2(0)\big)
\end{align*}
for all $j=1,\ldots, r$. Setting $\eta = \min\{\delta/4, 1/n\}$ and plugging the inequality above into the definition of $I_1$, we have that with probability at least $1-\delta/2$,
%\begin{align*}
%    \Bigg| \frac{1}{n} \sum_{i=1}^n U_{ij'} V_i - \EE(U_{1j'} V_1) \Bigg| \leq C_2 L\|\wb^*\|_2  \sqrt{\frac{2k\log(2n^2r)\log(60r/\delta)}{n}} + C_3\|\wb^*\|_2^2\frac{1}{\sqrt{n}}.
%\end{align*}
%Therefore we have
\begin{align}\label{eq:directionconcentrationOwtilde1}
    |I_1 - \EE[\zb^\top \tilde{\wb}] | \leq C_4 M' r  \sqrt{\frac{2k\log(2n^2r)\log(40r/\delta)}{n}}
\end{align}
for all $\zb \in \cN_{1/2}$, where $M' = \max\{ L[\|\wb^*\|_2 + |\sigma(0)|], \|\wb^*\|_2^2 + \sigma^2(0) \}$ and $C_4$ is an absolute constant.





\iffalse
\begin{align*}
    U^{(j)}_{ij'} &= [\sigma(\wb^{*\top}  \Pb_{j'} \xb_{i}) - \sigma(0)] \cdot \zb^\top\Pb_j\xb_i,\\
    V^{(j)}_{ij'} &= \sigma(0) \cdot \zb^\top\Pb_j\xb_i.
\end{align*}

By Lemma~\ref{lemma:subgaussianproduct} and (5.15) in \cite{vershynin2010introduction} as an equivalent definition of $\psi_1$-norm, we have 
$$
\|U^{(j)}_{ij'}\|_{\psi_1} \leq L\|\wb^{*\top} \Pb_{j'} \xb_{i} \cdot  \zb^\top\Pb_j\xb_i \|_{\psi_1} \leq  C_1L\|\wb^{*}\|,
$$
where $C_1$ is an absolute constant. Applying Proposition~5.16 in \cite{vershynin2010introduction} to $\{U^{(j)}_{ij'}\}$, we have that with probability at least $1-\delta/3$, we have
\begin{align*}
    \Bigg|\frac{1}{n} \sum_{i=1}^n U^{(j)}_{ij'} - \delta_{j,j'}\EE(\zb^\top \hat{\wb})\Bigg| \leq C_2L\|\wb^*\| \sqrt{\frac{k\log[30r^2/\delta]}{n}}
\end{align*}
for all $j,j'\in [r]$ and all $\zb \in \cN_{1/2}$, 
where $C_2$ is an absolute constant. Therefore with probability at least $1-\delta/3$, we have
\begin{align}\label{eq:directionconcentrationOwtilde1}
    \Big|I_1^{(j)} - \EE(\zb^\top \hat{\wb})\Big| \leq C_2Lr\|\wb^*\| \sqrt{\frac{k\log[30r^2/\delta]}{n}}
\end{align}
for all $j\in [r]$ and all $\zb \in \cN_{1/2}$.
\fi

\noindent \textbf{Concentration of $I_2$}. 
We have 
\begin{align*}
    I_2= \frac{1}{n} \sum_{i=1}^n \epsilon_{i}\cdot\zb^\top\Pb_1\xb_i.
\end{align*}
By Lemma~\ref{lemma:subgaussianproduct}, we have 
$\|\epsilon_{i}\cdot \zb^\top\Pb_1\xb_i\|_{\psi_1} \leq C_5 \nu$ for some absolute constant $C_5$. By Proposition~5.16 in \cite{vershynin2010introduction}, with probability at least $1-\delta/2$, we have
\begin{align}\label{eq:directionconcentrationOwtilde2}
    |I_2|  \leq C_6\nu \sqrt{\frac{k\log(20/\delta)}{n}}
\end{align}
for all $\zb\in \cN_{1/2}$, where $C_6$ is an absolute constant. 
By \eqref{eq:directionconcentrationOwtilde1}, \eqref{eq:directionconcentrationOwtilde2}, and the definition of $\tilde{\wb}$, we have
\begin{align*}
    \big|\zb^\top \big(\tilde{\wb} - \EE[\tilde{\wb}]\big)\big| \leq &  C_4 M' r  \sqrt{\frac{2k\log(2n^2r)\log(40r/\delta)}{n}} +  C_6\nu \sqrt{\frac{k\log(20/\delta)}{n}}
\end{align*}
for all $\zb\in \cN_{1/2}$. Now by Lemma~5.3 in \cite{vershynin2010introduction} and Lemma~\ref{lemma:momentcalculation}, we have that with probability at least $1-\delta$,
\begin{align*}
    \| \tilde{\wb} - \EE[\tilde{\wb}] \|_2 \leq & C\Bigg[M' r  \sqrt{\frac{2k\log(2n^2r)\log(40r/\delta)}{n}} +  \nu \sqrt{\frac{k\log(20/\delta)}{n}} \Bigg],
\end{align*}
where $C$ is an absolute constant. This completes the proof.



\iffalse
note that 
\begin{align*}
    \|\hat\wb-\EE[\hat\wb]\|_2^2\geq 2\|\hat\wb\|_2\cdot\|\EE[\hat\wb]\|_2-2\la\hat\wb,\EE[\hat\wb]\ra.
\end{align*}
It immediately implies that
\begin{align*}
    \bigg\la\frac{\hat\wb}{\|\hat\wb\|_2},\frac{\EE[\hat\wb]}{\|\EE[\hat\wb]\|_2}\bigg\ra\geq 1-\frac{1}{2\|\EE[\hat\wb]\|}\|\hat\wb-\EE[\hat\wb]\|_2^2
\end{align*}
\fi
\end{proof}



\begin{lemma}\label{lemma:directionconcentrationO}
In Algorithm~\ref{alg:OCNN}, we have
\begin{align*}
    \bigg\| \hat{\wb} - \frac{\gamma(\|\wb^*\|)}{\|\wb^*\|} \wb^* \bigg\|_2 &\leq C\Bigg[M' r  \sqrt{\frac{2k\log(2n^2r)\log(40r/\delta)}{n}} +  \nu \sqrt{\frac{k\log(20/\delta)}{n}} \Bigg], \text{ and}\\
    \bigg\la \frac{\hat{\wb}}{\|\hat{\wb}\|_2}, \frac{\wb^*}{\|\wb^*\|_2} \bigg\ra &\geq 1- \frac{C'}{\gamma^2(\|\wb^*\|_2)}  \Bigg[M' r  \sqrt{\frac{2k\log(2n^2r)\log(40r/\delta)}{n}} +  \nu \sqrt{\frac{k\log(20/\delta)}{n}} \Bigg]^2,
\end{align*}
where $M' = \max\{ L(\|\wb^*\|_2 + |\sigma(0)|), \|\wb^*\|_2^2 + \sigma^2(0) \}$, and $C, C'$ are absolute constants.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lemma:directionconcentrationO}]
Let
\begin{align*}
    \Ab = \begin{bmatrix}
    1       & 0 & 0 &  \dots & 0  & 0 \\
    -1       & 1 & 0 &  \dots & 0  & 0 \\
    0       & -1 & 1 &  \dots & 0  & 0 \\
    \hdotsfor{6}\\
    0       & 0 & 0 & \dots & 1  & 0 \\
    0       & 0 & 0 & \dots & -1  & 1 
\end{bmatrix} \in \RR^{k\times k}.
\end{align*}
Then in Algorithm~\ref{alg:OCNN} we have $\hat{\wb} = \Ab\tilde{\wb}$. Moreover by Lemma~\ref{lemma:directionconcentrationOwtildeexpectation}, we have
\begin{align*}
    \EE[\Ab\tilde{\wb}] = \frac{\gamma(\|\wb^*\|_2)}{\|\wb^*\|_2} \wb^*.
\end{align*}
Therefore,
\begin{align}\label{eq:directionconcentrationO1}
    \bigg\| \hat{\wb} - \frac{\gamma(\|\wb^*\|_2)}{\|\wb^*\|_2} \wb^* \bigg\|_2 \leq \| \Ab \|_2 \| \tilde{\wb} - \EE[\tilde{\wb}] \|_2
\end{align}
Note that we have
\begin{align*}
    \Ab^\top \Ab= \begin{bmatrix}
    2       & -1 & 0 &  \dots & 0  & 0 \\
    -1       & 2 & -1 &  \dots & 0  & 0 \\
    0       & -1 & 2 &  \dots & 0  & 0 \\
    \hdotsfor{6}\\
    0       & 0 & 0 & \dots & 2  & -1 \\
    0       & 0 & 0 & \dots & -1  & 1 
\end{bmatrix}.
\end{align*}
Therefore $\|\Ab\|_2$ is bounded by an absolute constant. The result of Lemma~\ref{lemma:directionconcentrationO} follows by \eqref{eq:directionconcentrationO1}, Lemma~\ref{lemma:directionconcentrationOwtilde} and Lemma~\ref{lemma:distance2innerproduct}.
\end{proof}




